Investigations into Proof Structures

We introduce and elaborate a novel formalism for the manipulation and analysis of proofs as objects in a global manner. In this first approach the formalism is restricted to first-order problems characterized by condensed detachment. It is applied in an exemplary manner to a coherent and comprehensive formal reconstruction and analysis of historical proofs of a widely-studied problem due to {\L}ukasiewicz. The underlying approach opens the door towards new systematic ways of generating lemmas in the course of proof search to the effects of reducing the search effort and finding shorter proofs. Among the numerous reported experiments along this line, a proof of {\L}ukasiewicz's problem was automatically discovered that is much shorter than any proof found before by man or machine.

==> img7/cmproof_expanded_02_xy.tex <==
\matrix[column sep=0.5em,row sep=0.4em] (m1) at (14.700000000000001,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{1}\\[\cmfiginl]
   \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_1y_1\\
   \& \rule[-1ex]{0pt}{3ex}\f{P}x_1\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_1\&\rule[-1ex]{0pt}{3ex}\f{P}g\nhphantom{$\f{P}g$}\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m2) at (12.25,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{2}\\[\cmfiginl]
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_1 \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_2y_2\\
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_2 \& \rule[-1ex]{0pt}{3ex}\f{P}x_2\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_2\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m3) at (9.8,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{3}\\[\cmfiginl]
   \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_3y_3\\
   \& \rule[-1ex]{0pt}{3ex}\f{P}x_3\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_3\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m4) at (7.3500000000000005,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{4}\\[\cmfiginl]
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_3 \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_4y_4\\
   \& \rule[-1ex]{0pt}{3ex}\f{P}x_4\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_4\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m5) at (4.9,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{5}\\[\cmfiginl]
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_4 \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_5y_5\\
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_5 \& \rule[-1ex]{0pt}{3ex}\f{P}x_5\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_5\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m6) at (2.45,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{6}\\[\cmfiginl]
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_6 \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_6y_6\\
   \& \rule[-1ex]{0pt}{3ex}\f{P}x_6\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_6\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m7) at (0.0,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{7}\\[\cmfiginl]
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_7 \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_7y_7\\
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_8 \& \rule[-1ex]{0pt}{3ex}\f{P}x_7\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_7\\
};

\draw[] (m1-4-2) edge node [midway,above] {\cmfigconn{1}} (m1-4-3);
\draw[] (m1-2-2.west) edge[in=85,out=220,looseness=1.1] node [pos=0.4,left] {\cmfigconn{2}} (m2-4-2.east);
\draw[] (m1-3-2.west) edge[in=-40,out=250,looseness=1.1] node [midway,above] {\cmfigconn{3}} (m3-4-2.east);
\draw[] (m2-2-1) edge node [midway,above] {\cmfigconn{4}} (m2-2-2);
\draw[] (m2-3-1) edge node [midway,above] {\cmfigconn{5}} (m2-3-2);
\draw[] (m3-2-2.west) edge[in=85,out=220,looseness=1.1] node [pos=0.4,left] {\cmfigconn{2}} (m4-4-2.east);
\draw[] (m3-3-2.west) edge[in=-40,out=250,looseness=1.1] node [midway,above] {\cmfigconn{3}} (m6-4-2.east);
\draw[] (m4-2-1) edge node [midway,above] {\cmfigconn{4}} (m4-2-2);
\draw[] (m4-3-2.west) edge[in=-40,out=250,looseness=1.1] node [midway,above] {\cmfigconn{3}} (m5-4-2.east);
\draw[] (m5-2-1) edge node [midway,above] {\cmfigconn{4}} (m5-2-2);
\draw[] (m5-3-1) edge node [midway,above] {\cmfigconn{5}} (m5-3-2);
\draw[] (m6-2-1) edge node [midway,above] {\cmfigconn{4}} (m6-2-2);
\draw[] (m6-3-2.west) edge[in=-40,out=250,looseness=1.1] node [midway,above] {\cmfigconn{3}} (m7-4-2.east);
\draw[] (m7-2-1) edge node [midway,above] {\cmfigconn{4}} (m7-2-2);
\draw[] (m7-3-1) edge node [midway,above] {\cmfigconn{5}} (m7-3-2);

